Craig Interpolation for Guarded Fragments

We show that the guarded-negation fragment (GNFO) is, in a precise sense, the smallest extension of the guarded fragment (GFO) with Craig interpolation. In contrast, %we show that the smallest extension of the two-variable fragment (FO2) with Craig interpolation is full first-order logic.

==> old/old-text.tex <==
\newpage
\hspace*{1pt} \newpage
\jesse{To-do: remove/move this}

We say that a fragment is \textit{closed under guarded quantification} if it can express $\exists \overline{x} (\alpha \land \varphi)$ whenever it can express $\varphi$, and a fragment is \textit{closed under guarded negation} if it can express $\alpha \land \lnot \varphi$ whenever it can express $\varphi$ (where $\alpha$ is an atomic formula and $free(\varphi)\subseteq free(\alpha)$).

An alternative characterization for \GNFO is that it is the logic which can express every union of conjunctive queries (UCQ) and is closed under guarded negation. This is made explicit in the following equivalent grammar for \GNFO:
$$\varphi := R(\overline{x}) \mid x = y \mid \alpha \land \lnot \varphi \mid q[\varphi_1 / R_1, \hdots, \varphi_n / R_n],$$
where $q$ is a UCQ with relation symbols $R_1, \hdots, R_n$ and $\varphi_1, \hdots, \varphi_n$ are self-guarded formulas with the appropriate number of free variables and generated by the same recursive grammar. We refer to this as the \textit{UCQ syntax} for \GNFO. The main thrust of our argument is to exploit this fact, showing first that

The ``minimal closure properties" in the above proposition are the expressibility of atomic formulas, conjunction, guarded quantification, and unary implication. For this last property, we say that a language can express unary implications if it can express $\alpha \to \phi$ whenever it can express $\phi$, where $\alpha$ is an atomic formula with only one free variable.

It is worth reflecting on these constraints for our arbitrary language $L$ extending \GFO. Given that \GFO is closed under conjunction, it is natural to confine attention to extensions which are also closed under conjunction. The more interesting constraints are that $L$ is be closed under unary implication and guarded quantification. As it turns out, these properties are consequences of a number of natural syntactic constructions. $L$ is easily seen to be closed under unary implications given any of the following conditions:
\begin{itemize}
  \item $L$ is closed under implication,
  \item $L$ is closed under unary negation and disjunction, or
  \item $L$ is closed under guarded negation and disjunction.
\end{itemize}
\textcolor{red}{In the case of guarded logics, we expect that the syntax ought to be closed under uniform substitutions of self-guarded formulas. We say that any such logic is \textit{closed under self-guarded substitutions}. Thus any guarded logic capable of expressing atomic existential formulas, those of the form $\exists \overline{x} \alpha$ for some atomic formula $\alpha$, is naturally closed under guarded quantification.} We thus settle on the following closure properties for our abstract logic $L$:
\begin{enumerate}[leftmargin=1.5cm,label={(\bfseries L\arabic*):}]
  \item $L$ can express all self-guarded \GFO-formulas;
  \item $L$ can express all atomic existential formulas;
  \item $L$ can express conjunction and disjunction;
  \item $L$ is closed under self-guarded substitution;
  \item $L$ satisfies CIP.
\end{enumerate}
It is worth noting that \GFO satisfies $(\textbf{L1})$-$(\textbf{L4})$, while $\GNFO$ satisfies $(\textbf{L1})$-$(\textbf{L5})$. From these properties, $L$ can express guarded negation, and thus meets the ``minimal closure properties'' of Theorem \ref{prop:CQs}. Then by closure under disjunction, $L$ can express all unions of conjunctive queries, from which our main theorem easily follows.
